Adaptability of Neural Networks on Varying Granularity IR Tasks

Recent work in Information Retrieval (IR) using Deep Learning models has yielded state of the art results on a variety of IR tasks. Deep neural networks (DNN) are capable of learning ideal representations of data during the training process, removing the need for independently extracting features. However, the structures of these DNNs are often tailored to perform on specific datasets. In addition, IR tasks deal with text at varying levels of granularity from single factoids to documents containing thousands of words. In this paper, we examine the role of the granularity on the performance of common state of the art DNN structures in IR.

==> Network_Structures.tex <==
\section{Network Architectures}
\subsection{Convolutional Neural Networks}
CNNs 

And when stacked, they are able to produce increasingly abstract representations of the information~\cite{lecun}. 
TODO
\subsection{Recurrent Neural Networks}
TODO
